Methods for the Reduction of Three-Loop QCD Form Factors

In this thesis, we study the three-loop QCD form factors. After an introduction and a discussion of the physics motivation, we generate the quark form factor using Qgraf. We then show how to bring the Feynman integrals into a unique form by using various trivial symmetries such as shifts in loop momenta. We then try (and fail) to reduce it to master integrals using the Laporta algorithm. After a discussion of our implementation of the Laporta algorithm (called "Solve") we perform an extensive classification of all the integrals into irreducible, reducible and loop-by-loop integrable topologies. We devise methods to deal with each of these cases. We show that our reduction code fails to reduce only a small set of 11 topologies. We finally give some partial results, and in the appendix we collect some already known master integrals.

==> title.tex <==
\begin{titlepage}
\selectlanguage{german}
\begin{center}
\title{Methods for the Reduction of the\\Three-Loop QCD Quark Form Factor}
\author{B.T\"odtli}

\vspace{4.0cm}

{\LARGE Doktorarbeit}\\[0.5cm]
\Large
der Mathematisch-naturwissenschaftlichen Fakult\"at\\[0.5cm]

der Universit\"at Z\"urich\\[2.5cm]

vorgelegt von\\[0.5cm]

{\LARGE Beat T\"odtli}\\[6.0cm]
\today\\[1.7cm]
Leiter der Arbeit:\\[0.5cm]
Prof.~Dr.~T.~Gehrmann\\[0.5cm]
Institut f\"ur theoretische Physik, Universit\"at Z\"urich

\end{center}
\end{titlepage}
\selectlanguage{british}

